Dataflow Analysis-Inspired Deep Learning for Efficient Vulnerability Detection

Deep learning-based vulnerability detection has shown great performance and, in some studies, outperformed static analysis tools. However, the highest-performing approaches use token-based transformer models, which are not the most efficient to capture code semantics required for vulnerability detection. Classical program analysis techniques such as dataflow analysis can detect many types of bugs based on their root causes. In this paper, we propose to combine such causal-based vulnerability detection algorithms with deep learning, aiming to achieve more efficient and effective vulnerability detection. Specifically, we designed DeepDFA, a dataflow analysis-inspired graph learning framework and an embedding technique that enables graph learning to simulate dataflow computation. We show that DeepDFA is both performant and efficient. DeepDFA outperformed all non-transformer baselines. It was trained in 9 minutes, 75x faster than the highest-performing baseline model. When using only 50+ vulnerable and several hundreds of total examples as training data, the model retained the same performance as 100% of the dataset. DeepDFA also generalized to real-world vulnerabilities in DbgBench; it detected 8.7 out of 17 vulnerabilities on average across folds and was able to distinguish between patched and buggy versions, while the highest-performing baseline models did not detect any vulnerabilities. By combining DeepDFA with a large language model, we surpassed the state-of-the-art vulnerability detection performance on the Big-Vul dataset with 96.46 F1 score, 97.82 precision, and 95.14 recall. Our replication package is located at https://doi.org/10.6084/m9.figshare.21225413 .

==> content_template.tex <==

\section{Submission of conference papers to ICLR 2023}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2023 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2023_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2023_conference.sty+ and \verb+iclr2023_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2023_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.


==> figures-tex/cfg.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.3\textwidth]{figures/cfg.pdf}
    \caption{{\tool} input: CFG + abstract dataflow embedding}
    \label{fig:cfg}
\end{figure}

==> figures-tex/runtime-2col.tex <==
\setcounter{table}{3}
\begin{table*}[ht!]
% \begin{table}[h]
% \centering
% \caption{Runtime and size of the different models.
% }\label{fig:runtime-size-comparison}
% \begin{subtable}[t]{\textwidth}
\centering
\caption{{\tool}'s training/inference time was faster than the baselines.}\label{runtime}
\begin{tabular}{|l||r|r|r|r|}
\hline
Model & \makecell[r]{Train time\\(ms)} & \makecell[r]{GPU Inference\\(ms/example)} & \makecell[r]{CPU Inference\\(ms/example)} & MACs/example \\
\hline\hline
LineVul         & 10h19m  & 11.06 & 1068.2 & 48.32 B  \\\hline
{\tool+LineVul} & 10h40m  & 15.36 & 1571.5 & 48.32 B  \\\hline %249,734,276
\hey{UniXcoder} & \hey{11h16m} & \hey{9.49} & \hey{486.0} & \hey{48.32 B}  \\\hline
\hey{\tool+UniXcoder} & \hey{13h22m} & \hey{13.29} & \hey{922.1} & \hey{48.32 B}  \\\hline
% UniXcoder         &   &  &  &   \\\hline
% CodeT5         &   &  &  &   \\\hline
{\tool}         & \textbf{9m}     & \textbf{4.64} & \textbf{5.8} & \textbf{40.27 M}      \\\hline
% {UniXcoder+LineVul} &   &  &  & \textcolor{red}{XXX} B  \\\hline
% {CodeT5+LineVul} &   &  &  & \textcolor{red}{XXX} B  \\\hline
\end{tabular}
% \end{subtable}
\end{table*}

==> trash.tex <==
\begin{removeenv}
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/embedding.png}
    \caption{Abstract dataflow embedding generation}
    \label{fig:embedding}
\end{figure}

\subsection{Embedding Semantic Features}
\label{sec:input-representation}
We used program semantic features of dataflow information (more specifically the reaching definitions) to represent a node. To represent the definitions that 




Based on domain knowledge of the root causes of bugs involving reaching definitions, we extracted several properties which are important in representing a single definition.

\begin{itemize}
    \item API calls: the calls to functions used in the definition.
    \item Data type: the data type of the variable being assigned.
    \item Constant: the constant values assigned in the definition.
    \item Operator: the operators used in the definition.
\end{itemize}

We designed {\it global dataflow embedding}

\bent{
We addressed these differences by developing an \textit{abstract dataflow embedding}, a one-hot encoding{{\needcite}} based on domain knowledge of the reaching definition problem. The one-hot encoding allows the neural network to represent discrete information, and domain knowledge is used to generalize the concrete dataflow information to programs outside the training dataset.
}

% \todo{Make it more complete.}



% For each CFG node which is a definition, we disassembled it into these properties.
We extracted these properties from every definition in the training dataset.
Because of the explosive nature of program identifiers \citep{karampatsis_big_2020}, there can be a potentially infinite number of unique values for each property; we counted the most frequent $k$ values for each property based on the training dataset and defined the threshold $k$ as a hyperparameter. If the property's value was not in the top-$k$, we used an UNKNOWN token to represent its value\bent{; if the property is not present in the definition, we used a NONE token}.
Finally, we assigned an embedding key to each property value and concatenated all the property embeddings to create the abstract dataflow embedding.

Figure \ref{fig:embedding} describes our approach with an example definition: \texttt{str = malloc(10 * argc)}. The four tables list, for each property, \bent{the NONE and UNKNOWN tokens and the most frequent 3 values that might appear in a dataset ($k = 3$)}.
\wip{
We denote the one-hot vector as a vector $\mathbb{N}^{n}$, where each element $i. 1 < i < k+2$ is the index of the bit which is set to 1.
}
Our framework extracts the 4 properties from the definition and converts them to embedding keys which are generated based on the training dataset, then concatenates the 4 property embeddings to form the abstract dataflow embedding.
\wip{
The resulting abstract embedding of $n_3$ is $\irow{3 & 2 & 4 & 4}$; this is different from that of $n_1$, which is $\irow{3 & 0 & 0 & 2}$ according to the same embedding keys (not shown), so the network represents the two nodes differently while also representing the common datatype.
The abstract dataflow embedding is not 100\% precise, so in some cases two different definitions are represented using the same embedding.
}

\wip{
Contrasted with the concrete embedding for $n_3$, which is $\irow{0 & 1}$, the abstract embedding is larger (5x4 elements), but is still a fixed size, so it will scale to any size dataset without impacting the model's efficiency. The embedding keys have consistent meanings among all programs in the dataset because each key represents one value of one property, which is not possible with the original DFA bit vector.
}

    
\end{removeenv}

\begin{wipenv}
We cannot direclty use this because:

Challenge (1): One key difference between DFA and GNN is that
DFA represents dataflow information as a discrete bit vector, while most GNN representations are fundamentally continuous\citep{bengio_representation_2012}.
% 
Challenge (2): Another key difference is that the information represented in the solution of a dataflow problem is unique in size and content to a specific program, while the input representation for a GNN must be a fixed size to work with most model architectures, and must generalize over many programs, including programs not in the training dataset.

In Section 3.3, we present our abstract dataflow embedding that addresses the challenges.
\end{wipenv}


\begin{removeenv}
\ben{Remove below, move full specification of reaching definition to appendix \ref{sec:dataflow-appendix}}

\noindent {\bf An Example}: Figure \ref{fig:overview} shows an example of how reaching definitions can be used to detect a potential null-pointer dereference bug.
The assignment \texttt{str = NULL} is usually overwritten by the heap allocation \texttt{str = malloc(10 * argc)}, which defines a non-null value and can be dereferenced at \texttt{str[(10 * argc)-1]} without error.
However, when \texttt{argc <= 1}, the definition \texttt{str = NULL} reaches the dereference, resulting in a segmentation fault.
$\bigcup$ is used as the meet operator so that the statement after a conditional incorporates the possible values from both branches.

To perform this analysis, the one can propagate the definitions which are ``generated'' along the control flow of the program and mark a definition as ``killed'' when another definition overwrites the variable.
% 

\begin{wipenv}
Figure \ref{fig:overview} shows a null-pointer dereference bug which can be detected with reaching definition analysis.
The assignment $n_1$: \texttt{str = NULL} is usually overwritten by the non-null heap allocation $n_3$: \texttt{str = malloc(10 * argc)} and dereferenced without error at $n_4$: \texttt{str[(10 * argc)-1]}.
However, when \texttt{argc <= 1}, the null definition \texttt{str = NULL} reaches the dereference, resulting in a segmentation fault.

\end{wipenv}

Concretely, the analysis uses the following specification:

\begin{itemize}
    \item Domain: $P = \{1, 0\}^D$ where $D$ is the number of variable definitions in the program.
    \item Meet operator: ${\meet}(v) = \bigcup_{u \in pred(v)} u$.
    \item Transfer function: ${\transfer}(v) = GEN[v] \cup (\sqcap_{u \in pred(v)}[u] - KILL[v])$, where:
    \begin{itemize}
        \item $GEN[v]$ is the set of definitions assigned in $v$ and
        \item $KILL[v]$ is the set of definitions which assign to the same variable as a variable assigned in $v$; these definitions are \textit{killed} and will no longer be relevant after $v$ assigns a new value to the variable.
    \end{itemize}
    \item Initial states $P^0_v = [0]^D \forall v \in V$.
    \item Direction $d = \text{forward}$.
\end{itemize}

To draw a parallel between the Kildall method used to perform DFA and the message-passing algorithm used to train graph neural networks, we designed node embedding as follows
\end{removeenv}


\begin{removeenv}
\ben{Move to appendix}
One minor difference between the two algorithms is that DFA iterates until it reaches a fixpoint, while GNN performs a fixed number of iterations.
\citet{kam_monotone_1977} showed that DFA converges within $d(G) + 3$ passes, where $d$ is the loop connectedness of $G$.
We set the hyperparameter $t$ based on the best validation performance through our experimentation (see Section \ref{sec:training-appendix}). \ben{Note, we did not rigorously set $t$ based on the best validation performance - we only set a value 1000 based on experimentation with values 10, 100, 1000, 5000, 10000.}
\end{removeenv}



\begin{removeenv}
\mycomment{
This propagation of dataflow on the CFG in dataflow algorithm is analogous to graph learning. As shown on the right of Figure~\ref{fig:analogy},Graph neural networks, for each node $v$, iteratively {\aggregate} information from neighboring nodes (Equation \ref{equ:aggregate}), then {\update} the information at that node (Equation \ref{equ:update}).
}
\ben{Remove - redundant}
For GNN, in each iteration, for each node $v$, the {\aggregate} function aggregates and transforms the information present in all neighbors of $v$, similar to ${\meet}$. Then, the {\update} function updates the information of $v$, similar to ${\transfer}$.
\wip{$f$ defines GEN and KILL based on the variable defined in the statement, which can be incorporated as learned priors in the {\aggregate} function.}
% In the GGNN architecture, the {\aggregate} and {\update} functions are learned by neural networks based on the data.
We designed {\tool} to follow the same algorithm as the generic Kildall method, but did not specify the {\aggregate} and {\update} functions so that during training, the model could learn functions which apply to the concrete dataflow problem.
\ben{Repeated, which one intended to keep?}
\end{removeenv}

The graph learning then uses {\it \aggregate} and \textit{\update} functions to compute and propagate the encoded dataflow information in the CFG, 


We designed {\tool} to follow the same algorithm as the generic Kildall method, but did not specify the {\aggregate} and {\update} functions so that during training, the model could learn functions which apply to the concrete dataflow problem. 


Similarly, in graph learning, we first construct a CFG of program. Our node embedding encodes dataflow information of $IN(v)$, $OUT(v)$, $GEN(v)$ and $KILL(v)$. 

\begin{wipenv}
 we propose our approach: {\tool}, shown in Figure \ref{fig:overview}.
First, we convert the source code to a CFG and annotate it with the abstract dataflow embedding, shown in detail in Figure \ref{fig:embedding}.

Finally, the representation output by graph learning can be used for vulnerability detection, or used to augment another model's representation (as we do in Section \ref{sec:effectiveness}).
\end{wipenv}
% \input{sections/abstract}


% Motivated by the causal relationship between bugs and dataflow analysis, we present {\tool}, \wip{a semantic feature extraction approach and embedding technique} for graph neural networks which is guided by dataflow analysis.
% We show that our approach is a performant and efficient feature representation for vulnerability detection. non-transformer-based vulnerability detection models while only taking \wip{13} minutes to train and having fewer than \wip{48k} parameters, and, in combination with the recent state-of-the-art transformer model, improves the state-of-the-art performance to \wip{96.4} F1 score


% We also investigate the level to which our model employs dataflow analysis in learning the vulnerability detection task.
% {\tool} performs on average \wip{250}\% better than recent


%we show that {\tool} can be used with the top performed model to achieve the state of the art performance of vulnerability detection with \wip{96.4} F1 score.
%\wip{less computational resources, including training time and the number of trainable parameters}, and, in combination with the recent state-of-the-art transformer model, improves the state-of-the-art performance to \wip{96.4} F1 score.


% \input{sections/introduction}



%it is important to use vulnerability detection tools before releasing software.


% Previous: DFA computes the data usage patterns and relations in the control flow graph (CFG) of a program  and reports vulnerability based on its cause, i.e., whether the values and data relations collected from the program indicates the occurrence of the vulnerability conditions.

%CFG is also a program representation used by dataflow analysis to detect vulnerabilities\citep{cesare_bugalyzecom_2013,yamaguchi_modeling_2014,others}.

% \paragraph{\textbf{Our approach:}}
% We propose {\tool}, which emulates DFA for vulnerability detection using graph neural networks (GNN) to learn a transfer function $f$.
% Our abstract dataflow representation is lightweight and generalizes to unseen data by extracting the information which is important for dataflow analysis.

% First, we parse the source code to a CFG representation.
% Next, we initialize the node features attached to the CFG with our abstract dataflow embedding, described in Section \ref{sec:input-representation}.
% Next, we emulate the Kildall method for solving the reaching definition dataflow problem by performing message-passing on the CFG edges.
% Finally, the representation output by the graph learning stage can be used to perform classify functions as vulnerable/non-vulnerable, or used to augment another model's representation (as we do in Section 

% \begifigure}

% \paragraph{\textbf{Contributions:}}


%\wip{Yet it still achieve the second}

%{\tool} outperformed non-transformer-based approaches by \xxx\% on average while taking only {\xxx} minutes to train and having only {\xxx} parameters. By combining with the state-of-the-art model \citep{fu_linevul_2022}, {\tool} improved the performance to 0.96 F1 score, and improvement of \xxx\%.

% We believe that neural networks which incorporating dataflow information are a new paradigm of neural program analysis and will enable future developments with greater precision and deductive ability.

% \input{sections/related-work}


% However, their PrograML model does not explicitly capture the domain-specific information used by dataflow analysis and \wip{their applications were not downstream tasks of dataflow analysis. \todo{Is device mapping such an application?}}
% We developed an abstract dataflow embedding which captures the domain-specific information used by dataflow analysis and applied {\tool} directly to vulnerability detection, which is a well-established downstream task of dataflow analysis.

% abstract dataflow embedding  (Section \ref{sec:input-representation})
% \begin{itemize}
%     \item Learning a static analyzer from data
%     \item IR2Vec
%     \item A Machine-Learning Algorithm with Disjunctive Model for Data-Driven Program Analysis
%     \item Path-sensitive code embedding via contrastive learning for software vulnerability detection (ContraFlow). They did not distribute their code.
%     \item LineVD. They did not report function-level vulnerability detection performance, and we tried but could not reproduce their model for function-level vulnerability performance.
%     % \item PrograML. this work does not explicitly incorporate dataflow problem into the model, only positional embedding, while our abstract dataflow embedding is explicitly designed for the reaching definition problem.
% %     % \item Word embeddings and CodeBERT (contrast with absdf representation)
% %     % \item Graph representations (contrast with CFG-only GNN)
% \end{itemize}

% We address the problem of function-level vulnerability detection, in which the goal is to predict whether a given snippet of code is vulnerable (contains a vulnerability) or non-vulnerable.


% VulDeePecker \citep{li_vuldeepecker_2018} uses BiLSTM on slices considering data dependencies.
% SySeVR \citep{li_sysevr_2021} uses BiGRU on slices considering control and data dependencies.
% Draper \citep{russell_automated_2019} transforms source code into a grid representation and uses CNN and RF.
% ReGVD \citep{nguyen_regvd_2022} is a GNN-based approach which extracts structure based on co-occurrence rather than the graph representations used in program analysis.
% Our approach exploits the implicit graph structure of CFG used in program analysis to learn more meaningful representations of programs.

% Devign \citep{zhou_devign_2019} is a GNN-based approach which uses Code Property Graphs (CPG), combining AST, CFG, and PDG, annotated with Word2Vec \citep{mikolov_efficient_2013} embeddings.
% ReVeal \citep{chakraborty_deep_2021} is a GNN-based approach based on CPG which addresses class imbalance by using SMOTE and triplet loss.
% IVDetect \citep{li_vulnerability_2021} is a GNN-based approach which extracts the most important subgraph of the PDG as a fine-grained interpretation.
% LineVD \citep{hin_linevd_2022} is a GNN-based approach based on PDG  which combines statement-level and function-level CodeBERT embeddings; they did not report function-level metrics, and we could not reproduce their statement-level performance, so we did not report function-level performance from our reproduction.
% Our approach uses a lightweight abstract dataflow embedding rather than unsupervised embeddings, and uses CFG edges only because these are linked with DFA, making it more efficient.

% CodeBERT \citep{feng_codebert_2020} is a transformer model pretrained on a large body of NL-PL pairs, fine-tuned for vulnerability detection.
% LineVul \citep{fu_linevul_2022} is a transformer model based on CodeBERT which interprets the attention scores to produce line-level predictions.
% Our approach is pretrained only on program definitions in the dataset rather than an expensive pretraining phase, and connects only the meaningful edges in the CFG rather than each pair of tokens, making it more efficient than the transformer models.

% Devign \citep{zhou_devign_2019} uses GNN on Code Property Graphs (CPG), combining AST, CFG, and PDG, annotated with Word2Vec \citep{mikolov_efficient_2013} embeddings.
% ReVeal \citep{chakraborty_deep_2021} uses GNN on CPG and addresses class imbalance by using SMOTE and triplet loss.
% IVDetect \citep{li_vulnerability_2021} uses GNN on PDG with additional embeddings.
% LineVD \citep{hin_linevd_2022} uses GNN on PDG  annotated with statement-level and function-level CodeBERT embeddings.

% LineVD \citep{hin_linevd_2022} is a GNN-based approach based on PDG  which combines statement-level and function-level CodeBERT embeddings; they did not report function-level metrics, and we could not reproduce their statement-level performance, so we did not report function-level performance from our reproduction.

% \input{sections/background}


% \input{sections/method}


%A \textit{definition} is an expression which assigns a value to a variable, such as \texttt{p = NULL}. 

% In particular, one instance of dataflow analysis, called {\it reaching definition analysis}, aims to report at which program points, a particular variable definition can {\it reach}.

%gathering information about possible values throughout a program's execution.DFA is commonly used for program optimization or static analysis; one analysis, called reaching definitions, can be used for constant propagation or for detecting certain classes of bugs such as null-pointer dereferences.

%A simple approach of performing DFA is the {\it Kildall method} \citep{kildall_unified_1973}, an iterative algorithm which propagates information between neighbors in the CFG.This generic algorithm can be instantiated to detect different vulnerabilities based on the two dataflow equations the user specifies, including the \textit{meet operation} and \textit{update function}.

%The two together determine the type of program information and how it is propagated. 

% Here, each node is a statement {\it S}, and the edge indicates the order of execution between two statements.

% Dataflow analysis uses two equations to propagate the dataflow information through the neibouring nodes in the CFG, namely {\it meet operation} and {\it update function}.

%\todo{Check does GGNN use $AGGREGARTE^t$ or the same function $AGGREGATE$ for all $t$}
% We use $h^t_v$ to denote the information present at node $v$ at step $t$; $h^0_v$ denotes the initial node features.
%\todo{Ben please add the explanations for the notations}

% \todo{graph editing: add a title: (A) dataflow analysis (B) Graph Learning}



%and the information can be applied for program optimization or static analysis.

%\todo{Explain how reaching def transfer/meet works.}

% Dataflow analysis is a method for gathering information about possible values through points in a program's control-flow graph (CFG).
% Dataflow analysis is a method for gathering information about possible values throughout a program's execution.
% The information is commonly used for program optimization or static analysis; for example, reaching definitions can be used for constant propagation or for detecting certain classes of bugs such as null-pointer dereferences.

% Many dataflow analyses can be solved using the {\it fixpoint method \citep{the kildall method}} \todo{find the best term}, an iterative algorithm which propagates information between neighbors in the CFG.
% Ths generic algorithm is used to generate different kinds of information by specifying a \textit{transfer function} and \textit{meet operator}. In each iteration, for each node $v$, the meet operator combines the information of the neighbors of $v$, and the transfer function updates the information of $v$ to a new state reflecting the information of its neighbors. %\todo{Make it more complete and precise.}

% Let $G = (V, E)$ be a directed graph.
% $pred(v)$ denotes the predecessors of $v$.
% A data flow framework is specified with:

% \begin{itemize}
%     \item Domain $P$: the set of states which can be assigned to a program point. Commonly, this is represented with a bit vector.
%     \item Meet operator ${\meet}: P \times P \rightarrow P$: the operator used to aggregate multiple states which are propagated to a single node.
%     \item Transfer function ${\transfer}: V \times P \rightarrow P$: the function used to update the state of a single node at each iteration.
%     \item Initial states $P_0 \in V \times P$: the set of initial states for each node in the CFG.
%     \item Direction $d \in \{\text{forward}, \text{backward}\}$: whether to progress along (forward) or against (backward) the direction of the CFG edges.
% \end{itemize}

% In this paper, we apply to vulnerability detection the concrete problem of calculating \textit{reaching definitions}.
% %\todo{Explain how reaching def transfer/meet works.}
% Reaching definitions can be used to detect many bugs, such as null-pointer dereference, buffer overflow, double-free, and use-after-free bugs \citep{bugalyze}.
% A \textit{definition} is an expression which assigns a value to a variable name; the reaching definitions of a node are the definitions which are still assigned to that node without being overridden between the definition and the node.
% To solve this problem, one can propagate the definitions which are "generated" along the control flow of the program and mark a definition as "killed" when another definition overwrites the variable.
% We used the following specification:

% \begin{itemize}
%     \item Domain: $P = \{1, 0\}^D$ where $D$ is the number of variable definitions in the program.
%     \item Meet operator: ${\meet}(v) = \bigcup_{u \in pred(v)} u$.
%     \item Transfer function: ${\transfer}(v) = GEN[v] \cup (\sqcap_{u \in pred(v)}[u] - KILL[v])$, where:
%     \begin{itemize}
%         \item $GEN[v]$ is the set of definitions assigned in $v$ and
%         \item $KILL[v]$ is the set of definitions which assign to the same variable as a variable assigned in $v$; these definitions are \textit{killed} and will no longer be relevant after $v$ assigns a new value to the variable.
%     \end{itemize}
% \end{itemize}

% Our {\tool} approach draws a parallel between the fixpoint method used to solve dataflow problems and the message-passing algorithm used to train graph neural networks.


% \begin{figure}[t]
%      \centering
%      \begin{subfigure}{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/overview.png}
%          \caption{Overview of our {\tool} approach}
%          \label{fig:three sin x}
%      \end{subfigure}
%     %  \hfill
    
%      \begin{subfigure}{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/embedding.png}
%          \caption{Abstract dataflow embedding generation}
%          \label{fig:five over x}
%      \end{subfigure}
% \end{figure}


% \todo{Address differences.
% \begin{itemize}
%     \item DFA iterates until fixpoint while GNN uses a set number of iterations. It is known that DFA converges within a number of steps proportional to the depth of the CFG \needcite.
%     \item DFA GEN/KILL vs. GNN using neural networks: learned priors can incorporate GEN/KILL.
%     \item DFA discrete vs. GNN continuous: next section
% \end{itemize}
% }

% The {\aggregate} and {\update} iterations of GNN are similar to the meet operator (${\meet}$) and transfer function (${\transfer}$) specified in the fixpoint method.
% For GNN, in each iteration, for each node $v$, the {\aggregate} function aggregates and transforms the information present in all neighbors of $v$, similar to ${\meet}$. Then, the {\update} function updates the information of $v$, similar to ${\transfer}$.
% % In the GGNN architecture, the {\aggregate} and {\update} functions are learned by neural networks based on the data.
% We designed {\tool} to follow the same algorithm as the generic fixpoint method, but did not specify the {\aggregate} and {\update} functions so that the model could learn information which applies to the concrete dataflow problem.


% The information propagated by the fixpoint method is often represented as a discrete bit vector, while neural network representations are fundamentally continuous\citep{bengio}.
% % 
% Another key difference is that the information represented in the solution of a dataflow problem is restricted to a specific program, but the information learned in a neural network model should generalize over many programs.
% % 
% We addressed these differences by making {\tool}'s input representation a one-hot encoding{{\needcite}} based on domain knowledge of the concrete dataflow problem we targeted (reaching definition). The one-hot encoding allows the neural network to represent discrete information, and the domain knowledge is used to generalize the input representation to work over the whole dataset. \todo{Make it more complete.}

% Based on the parallel between DFA and GNN, we propose our approach: {\tool}, shown in Figure \ref{fig:overview}.
% First, we parse the source code to a CFG representation and initialize the node features with our abstract dataflow representation, described in Section \ref{sec:input-representation}.
% Next, during the graph learning stage, we emulate the fixpoint method for solving the reaching definition dataflow problem by performing message-passing on the CFG edges.
% Then, we read out the learned node-level representations to produce a graph-level representation.
% Finally, the graph-level representation can be used to predict a function-level binary classification, or used to augment another model's representation (as we do in Section \ref{sec:rq2}).
% \todo{Make an actual description}.

% \begin{itemize}
%     \item Parallel between dataflow and GNN.
%     Aggregate $\rightarrow$ meet operator.
%     Update $\rightarrow$ transfer function.
%     \item Differences?
%     \begin{itemize}
%         \item Discrete bit vector used in fixpoint, continuous in NN.
%         \item Single-program representation vs. whole dataset representation.
%         \item How did we address them?
%     \end{itemize}
% \end{itemize}

% The input is the source code of a potentially buggy program.
% Next, we perform graph learning to emulate the Kildall method for solving the reaching definition dataflow problem by performing message-passing on the CFG edges.
% First, we parse the source code to a CFG representation.
% Next, we initialize the node features attached to the CFG with our abstract dataflow embedding, described in Section \ref{sec:input-representation}.
% Next, we emulate the Kildall method for solving the reaching definition dataflow problem by performing message-passing on the CFG edges.
% Finally, the representation output by the graph learning stage can be used to perform classify functions as vulnerable/non-vulnerable, or used to augment another model's representation (as we do in Section \ref{sec:effectiveness}).

% Figure \ref{fig:overview} shows an example of how reaching definitions can be used to detect a potential null-pointer dereference bug.

% There are 4 nodes in the graph, $n_1$, $n_2$, $n_3$, $n_4$ and 2 definitions, $d_1$ and $d_2$.
% The domain is the bitset of all definitions in the program, in this case $\irow{d_1 & d_2}$ where each bit $d_i \in \{0, 1\}$ represents a definition.

% \frame{
% \begin{tikzpicture}
%     \begin{axis}[width=3 ex, height = 3 ex, 
%                  scale only axis, hide axis]
%         % \addplot[black] {rand};
%         \draw (0,0) rectangle node{$d1$} (2,2);
%     \end{axis};
% \end{tikzpicture}}

% One key difference between DFA and GNN is that the information propagated by DFA is represented as a discrete bit vector \wip{$v \in \{ 0, 1 \}^d$ for some fixed length $d$}, while most GNN representations are fundamentally continuous\citep{bengio_representation_2012}.
% A simple assignment \texttt{x = 0} can be harmless in one program and cause a null-pointer dereference bug in another program, even though the variable name and value assigned are the same.
% 
% Even a simple assignment \texttt{x = 0} can be dead code in one program and cause a null pointer error in another, even though the variable name and value assigned are the same.
% Also, similar definitions should be represented similarly in order for the network to learn to recognize bug patterns, in spite of small changes.
% 
%%%%% PREVIOUS DRAFT- copied for shortening
% One key difference between DFA and GNN is that the information propagated by DFA is represented as a discrete bit vector, while most GNN representations are fundamentally continuous\citep{bengio_representation_2012}.
% % 
% Another key difference is that the information represented in the solution of a dataflow problem is unique to a specific program.
% When calculating reaching definitions, each definition is unique within a single program because it must be interpreted in the context of that program, and the size of the bit vector is the number of definitions in the program.
% However, the input representation for a GNN must be a fixed size to work with most model architectures, and must generalize over many programs, including programs not in the training dataset
% 
% We addressed these differences by developing a one-hot encoding{{\needcite}} based on domain knowledge of the reaching definition problem. The one-hot encoding allows the neural network to represent discrete information, and our domain knowledge is used to generalize the input representation to programs outside the training dataset.
% We extracted the most important parts of the concrete definition and concatenated the different parts to make an \textit{abstract dataflow embedding}.
%%%%% PREVIOUS DRAFT- copied for shortening

% We designed the properties used in the embedding intending so that the embeddings would be mostly unique within a single program.

% The information propagated by the Kildall method is often represented as a discrete bit vector, while conventional neural network representations are fundamentally continuous\citep{bengio}.
% % 
% Another key difference is that the information represented in the solution of a dataflow problem is restricted to a specific program, but the information learned in a neural network model should generalize over many programs.
% % 
% We addressed these differences by making {\tool}'s input representation a one-hot encoding{{\needcite}} based on domain knowledge of the concrete dataflow problem we targeted (reaching definition). The one-hot encoding allows the neural network to represent discrete information, and the domain knowledge is used to generalize the input representation to work over the whole dataset. \todo{Make it more complete.}

% When calculating reaching definitions, each definition is unique within a single program because it must be interpreted in the context of that program. Even a simple assignment \texttt{x = 0} can be dead code in one program and cause a null pointer error in another, even though the variable name and value assigned are the same.
% Also, similar definitions should be represented similarly in order for the network to learn to recognize bug patterns, in spite of small changes.

% For dataflow problems, we initialize a different bit vector for each program, with one bit representing each definition in the program. However, graph neural networks require a fixed-size input representation, and a good representation should be consistent (each part of the input retains the same meaning) among all programs in the dataset.
% We developed an abstract dataflow input representation in order to fulfill these requirements.

% Based on domain knowledge of definitions, we developed several properties which are pertinent in representing a single definition. \todo{justify why these are the best properties.}
% \begin{itemize}
%     \item api calls: the calls to functions used in the definition.
%     \item data type: the data type of the variable being assigned.
%     \item literals: the literal values assigned in the definition.
%     \item operator: the operators used in the definition.
% \end{itemize}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/absdf.png}
%     \caption{Converting an example definition into the abstract input representation. \todo{show only one example, make it more compact and complete}}
%     \label{fig:absdf}
% \end{figure}

% We assigned an embedding key to each property and concatenated the property indices into an index for the node.
% Because of the explosive nature of program vocabularies \citep{program vocabulary representation}, there can be a potentially infinite number of unique values for each property; we counted the most frequent $k$ items in each property based on the training dataset and defined the threshold $k$ as a hyperparameter. If the property's value was not in the top-$k$, we used an UNKNOWN token to represent its value.

% For each node which is a definition, we disassembled it into these properties.
% Then, we assigned an index to each property and concatenated the property indices into an index for the node.
% Because of the explosive nature of program vocabularies \citep{program vocabulary representation}, there can be a potentially infinite number of unique values for each property; we counted the most frequent $k$ items in each property based on the training dataset and defined the threshold $k$ as a hyperparameter. If the property's value was not in the top-$k$, we used an UNKNOWN token to represent its value.

% Figure \ref{fig:absdf} describes our approach with an example definition: \texttt{char *ptr = malloc(1 * sizeof(int));}. The four tables list sample values for the UNKNOWN token and the most frequent 3 values that might appear in a dataset ($k = 3$).
% To convert the definition to its abstract dataflow representation, our framework extracts the 4 properties from the definition (if present), then indexes into the lookup tables which are generated based on the training dataset, and finally concatenates the 4 property encodings to form the input representation.

% \begin{itemize}
%     % \item Naive extraction method
%     \item Abstract dataflow
%     \item Vocabulary problem
% \end{itemize}



     
\mycomment{

Let $G = (V, E)$ be a directed graph.
$pred(v)$ denotes the predecessors of $v$.
A data flow framework is specified with:

\begin{itemize}
    \item Domain $P$: the set of states which can be assigned to a program point, commonly represented with a bit vector.
    \item Meet operator ${\meet}: P \times P \rightarrow P$: the operator used to aggregate the states of multiple predecessors at each iteration.
    % \item Meet operator ${\meet}: P \times P \rightarrow P$: the operator used to aggregate multiple states which are propagated to a single node.
    \item Transfer function ${\transfer}: V \times P \rightarrow P$: the function used to update the state of a single node at each iteration.
    \item Initial states $P^0 \in V \times P$: the set of initial states for each node in the CFG.
    \item Direction $d \in \{\text{forward}, \text{backward}\}$: whether to progress along (forward) or against (backward) the direction of the CFG edges.
\end{itemize}

We apply to vulnerability detection the concrete problem of calculating \textit{reaching definitions}.
Reaching definitions can be used to detect many bugs, such as null-pointer dereference, buffer overflow, double-free, and use-after-free bugs \citep{cesare_bugalyzecom_2013}.
A \textit{definition} is an expression which assigns a value to a variable name, such as \texttt{str = NULL}; the reaching definitions of a node are the definitions which are assigned to that node without having been overridden between the definition and the node.
% 
}

\mycomment{
\subsection{Graph Neural Networks} 

\begin{wipenv}
Graph neural networks\citep{graph networks deepmind} are trained with the message-passing algorithm (we adapt the formulation presented in \citep{gin}).
We use $h^t_v$ to denote the information present at node $v$ at step $t$; $h^0_v$ denotes the initial node features.
Graph neural networks, for each node $v$, iteratively {\aggregate} information from neighboring nodes (Equation \ref{equ:aggregate}), then {\update} the information at that node (Equation \ref{equ:update}).

\begin{equation} \label{equ:aggregate}
    a^t_v = {\aggregate}^t (\{ h^{t-1}_u | u \in pred(v) \})
\end{equation}

\begin{equation} \label{equ:update}
    h^t_v = {\update} (h^{t-1}_v, a^t_v)
\end{equation}

After a fixed number of iterations, the information from all nodes is combined with a graph readout operation to produce a graph-level classification.

\end{wipenv}

}


% \input{sections/method} old


%A \textit{definition} is an expression which assigns a value to a variable, such as \texttt{p = NULL}. 

% In particular, one instance of dataflow analysis, called {\it reaching definition analysis}, aims to report at which program points, a particular variable definition can {\it reach}.

% Next, we perform graph learning to emulate the Kildall method for solving the reaching definition dataflow problem by performing message-passing on the CFG edges.

%gathering information about possible values throughout a program's execution.DFA is commonly used for program optimization or static analysis; one analysis, called reaching definitions, can be used for constant propagation or for detecting certain classes of bugs such as null-pointer dereferences.

%A simple approach of performing DFA is the {\it Kildall method} \citep{kildall_unified_1973}, an iterative algorithm which propagates information between neighbors in the CFG.This generic algorithm can be instantiated to detect different vulnerabilities based on the two dataflow equations the user specifies, including the \textit{meet operation} and \textit{update function}.


%The two together determine the type of program information and how it is propagated. 

% First, we parse the source code to a CFG representation.
% Next, we initialize the node features attached to the CFG with our abstract dataflow embedding, described in Section \ref{sec:input-representation}.
% Next, we emulate the Kildall method for solving the reaching definition dataflow problem by performing message-passing on the CFG edges.
% Finally, the representation output by the graph learning stage can be used to perform classify functions as vulnerable/non-vulnerable, or used to augment another model's representation (as we do in Section \ref{sec:effectiveness}).

% Figure \ref{fig:overview} shows an example of how reaching definitions can be used to detect a potential null-pointer dereference bug.

% There are 4 nodes in the graph, $n_1$, $n_2$, $n_3$, $n_4$ and 2 definitions, $d_1$ and $d_2$.
% The domain is the bitset of all definitions in the program, in this case $\irow{d_1 & d_2}$ where each bit $d_i \in \{0, 1\}$ represents a definition.

% \frame{
% \begin{tikzpicture}
%     \begin{axis}[width=3 ex, height = 3 ex, 
%                  scale only axis, hide axis]
%         % \addplot[black] {rand};
%         \draw (0,0) rectangle node{$d1$} (2,2);
%     \end{axis};
% \end{tikzpicture}}

% One key difference between DFA and GNN is that the information propagated by DFA is represented as a discrete bit vector \wip{$v \in \{ 0, 1 \}^d$ for some fixed length $d$}, while most GNN representations are fundamentally continuous\citep{bengio_representation_2012}.
% A simple assignment \texttt{x = 0} can be harmless in one program and cause a null-pointer dereference bug in another program, even though the variable name and value assigned are the same.
% 
% Even a simple assignment \texttt{x = 0} can be dead code in one program and cause a null pointer error in another, even though the variable name and value assigned are the same.
% Also, similar definitions should be represented similarly in order for the network to learn to recognize bug patterns, in spite of small changes.
% 
%%%%% PREVIOUS DRAFT- copied for shortening
% One key difference between DFA and GNN is that the information propagated by DFA is represented as a discrete bit vector, while most GNN representations are fundamentally continuous\citep{bengio_representation_2012}.
% % 
% Another key difference is that the information represented in the solution of a dataflow problem is unique to a specific program.
% When calculating reaching definitions, each definition is unique within a single program because it must be interpreted in the context of that program, and the size of the bit vector is the number of definitions in the program.
% However, the input representation for a GNN must be a fixed size to work with most model architectures, and must generalize over many programs, including programs not in the training dataset
% 
% We addressed these differences by developing a one-hot encoding{{\needcite}} based on domain knowledge of the reaching definition problem. The one-hot encoding allows the neural network to represent discrete information, and our domain knowledge is used to generalize the input representation to programs outside the training dataset.
% We extracted the most important parts of the concrete definition and concatenated the different parts to make an \textit{abstract dataflow embedding}.
%%%%% PREVIOUS DRAFT- copied for shortening

% For each CFG node which is a definition, we disassembled it into these properties.

% We designed the properties used in the embedding intending so that the embeddings would be mostly unique within a single program.

% The information propagated by the Kildall method is often represented as a discrete bit vector, while conventional neural network representations are fundamentally continuous\citep{bengio}.
% % 
% Another key difference is that the information represented in the solution of a dataflow problem is restricted to a specific program, but the information learned in a neural network model should generalize over many programs.
% % 
% We addressed these differences by making {\tool}'s input representation a one-hot encoding{{\needcite}} based on domain knowledge of the concrete dataflow problem we targeted (reaching definition). The one-hot encoding allows the neural network to represent discrete information, and the domain knowledge is used to generalize the input representation to work over the whole dataset. \todo{Make it more complete.}

% When calculating reaching definitions, each definition is unique within a single program because it must be interpreted in the context of that program. Even a simple assignment \texttt{x = 0} can be dead code in one program and cause a null pointer error in another, even though the variable name and value assigned are the same.
% Also, similar definitions should be represented similarly in order for the network to learn to recognize bug patterns, in spite of small changes.

% For dataflow problems, we initialize a different bit vector for each program, with one bit representing each definition in the program. However, graph neural networks require a fixed-size input representation, and a good representation should be consistent (each part of the input retains the same meaning) among all programs in the dataset.
% We developed an abstract dataflow input representation in order to fulfill these requirements.

% Based on domain knowledge of definitions, we developed several properties which are pertinent in representing a single definition. \todo{justify why these are the best properties.}
% \begin{itemize}
%     \item api calls: the calls to functions used in the definition.
%     \item data type: the data type of the variable being assigned.
%     \item literals: the literal values assigned in the definition.
%     \item operator: the operators used in the definition.
% \end{itemize}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/absdf.png}
%     \caption{Converting an example definition into the abstract input representation. \todo{show only one example, make it more compact and complete}}
%     \label{fig:absdf}
% \end{figure}

% We assigned an embedding key to each property and concatenated the property indices into an index for the node.
% Because of the explosive nature of program vocabularies \citep{program vocabulary representation}, there can be a potentially infinite number of unique values for each property; we counted the most frequent $k$ items in each property based on the training dataset and defined the threshold $k$ as a hyperparameter. If the property's value was not in the top-$k$, we used an UNKNOWN token to represent its value.

% For each node which is a definition, we disassembled it into these properties.
% Then, we assigned an index to each property and concatenated the property indices into an index for the node.
% Because of the explosive nature of program vocabularies \citep{program vocabulary representation}, there can be a potentially infinite number of unique values for each property; we counted the most frequent $k$ items in each property based on the training dataset and defined the threshold $k$ as a hyperparameter. If the property's value was not in the top-$k$, we used an UNKNOWN token to represent its value.

% Figure \ref{fig:absdf} describes our approach with an example definition: \texttt{char *ptr = malloc(1 * sizeof(int));}. The four tables list sample values for the UNKNOWN token and the most frequent 3 values that might appear in a dataset ($k = 3$).
% To convert the definition to its abstract dataflow representation, our framework extracts the 4 properties from the definition (if present), then indexes into the lookup tables which are generated based on the training dataset, and finally concatenates the 4 property encodings to form the input representation.

% \begin{itemize}
%     % \item Naive extraction method
%     \item Abstract dataflow
%     \item Vocabulary problem
% \end{itemize}

% \input{sections/experiments}


%\ben{Dr. Le, this Evaluation section is ready for revision.I highlighted in red the sections for which I think the phrasing could be improved.The number values are the final results from my experiments - I highlighted all numbers in red so I can remember to double-check them after I export the data and reproducibility package.}


    % \item \wip{Is {\tool} \textbf{robust} to semantic-preserving changes?}
    
% \noindent{\bf Experimental setup and metrics}
% Effectivness:accuracy, recall, F1
 
% model size and learning time

% generalization: across project, across bug types 

% Reduction cross-project vs mixed-project

%We created another setting of {\tool} by 

%For \textbf{{\tool}}, we used the GGNN model  as the model architecture for {\tool}.
% \wip{This architecture trains a GRU as the {\update} function and MLP as the {\aggregate} functions, and uses Global Attention Pooling for readout.}
%For \textbf{{\combinedtool}}, we concatenated LineVul's RoBERTa encoder output to {\tool}'s graph stage output after readout.
% , which are capable of learning the fixpoint method to solve the dataflow problem

% \wip{
% To avoid data leakage, we trained the abstract dataflow input representation on training set from the LineVul split.

%We trained the models on the {\dataset} dataset , which consists of vulnerable and non-vulnerable functions from real-world open-source C/C++ projects.The dataset contains 188,636 functions, of which 10,900 (6\%) are labeled vulnerable.\wip{This reflects the imbalanced distribution of real-world code, with the minority of code containing vulnerabilities \needcite.}

% {\dataset} dataset. LineVul splits (except numbers reported from IVDetect paper).
% Imbalanced.
% train/valid/test split.

%dataand our prototype implementation of the abstract dataflow representation does not handle all C language features, \wip{7\%} of programs in the {\dataset} dataset could not be handled by {\tool}. To ensure a fair comparison, these examples were excluded from training/validation/testing for the models in Table \ref{fig:compare-transformer}. The missing examples are an artifact of our research prototype, which can be improved by introducing a better parser and improving the abstract dataflow implementation.


% We chose this tool because it is able to parse C code without compiling it, using island parsers.
% Since the tool is implemented in Scala, it has low performance and overhead during startup/shutdown of the REPL; Our implementation extends the tool with a session-based script, cutting down on the startup/shutdown time.



% \begin{wraptable}{rh}{0.65\linewidth}
% \caption{Five Types of Vulnerabilities}
% \begin{center}
%  %\resizebox{0.96\columnwidth}{!}{
% \begin{tabular}{|l||c|c|}
% \hline
% Vulnerability Type             & Total &  CWE examples  \\\hline\hline
% Buffer overflow & 37,691 & CWE-125, CWE-787\\\hline
% Value error & 15,126 & CWE-190, CWE-369\\\hline
% Resource error & 33,748 & CWE-415, CWE-404\\\hline
% Input validation error & 25,514 & CWE-134, CWE-89\\\hline
% Privilege escalation & 32,749 & CWE-264, CWE-255\\\hline\hline 
% All bug types & 144,828 & - \\\hline 
% \end{tabular}
% %}
% \label{bugtype}
% \end{center}
% \end{wraptable}

%\ben{Let's move these details to appendix if we need space.}
% To study the generalization performance, we prepared cross-project and cross-bugtype test partitions of the {\dataset} dataset.
\begin{mycomment}{
To study generalization to unseen projects, we prepared a cross-project test dataset made of projects which are distinct from the training dataset.
Different projects use different style, language features, and naming conventions which may make it difficult for models to generalize.
To make the cross-project test dataset, we held out 10k examples from randomly selected projects in {\dataset}, ensuring projects represented in the cross-project dataset were mutually exclusive from the remaining data. Then we randomly partitioned the remaining data into train/validation/test sets with 10k examples in the validation and test data, and the remaining examples in training; one project may be represented by examples in the training and test dataset, so we call this the mixed-project test dataset.
To mitigate the effect of the selection of projects, we repeated this process 5 times with different selections of the cross-project dataset to perform 5-fold cross validation.
% To make the cross-bugtype dataset, we split the dataset into 5 bugtype datasets based on groups of CWEs. We partitioned each bugtype dataset into train/validation/test sets with 80/10/10\% portions. The details of the generation are listed in Section \ref{sec:generalization-dataset-appendix}.

% \begin{wipenv}
% \todo{Semantic-preserving changes}
% \begin{itemize}
%     \item Which changes and why they were chosen
%     \item Why it matters
% \end{itemize}
% \end{wipenv}

% Copypaste from empirical paper below

% In the second experiment, we prepared a {\it mixed-projects} setting where the test set is separated from the training set without considering the source project, and some examples in the training and test sets may originate from the same projects. This is the setting where most of our deep learning papers are evaluated with. We also constructed a {\it cross-projects} setting where the test set examples must originate from different projects than the projects represented the training set. This setting helps us understand whether we will have a significant performance degradation when using an off-the-shelf trained deep learning vulnerability detection models that have not seen the test projects.

% %\wip{
% We also used the {\dataset} dataset in a 5-fold cross validation setting. For each fold, we first constructed a test set for the cross-project setting by including all the examples from randomly chosen projects, until the set contained at least 10k examples. Because each project had a different number of examples, the resulting set was slightly larger than 10k examples. We then constructed a test set for the mixed-project setting by randomly partitioning the remaining examples into test (10 k), validation (10 k), and training (the remaining examples, about 158 k) sets.  We trained the model, using the 158 k training examples and 10 k validation set, then ran it on the test sets for both the cross-project setting and the mixed-project setting.
}
\end{mycomment}

\mycomment{
\begin{itemize}
    \item \textbf{Precision}, the portion of positive predictions which were correct: $P = \frac{TP}{TP+FP}$.
    \item \textbf{Recall}, the portion of positive examples which were recalled: $R = \frac{TP}{TP+FN}$.
    \item \textbf{F1}, the harmonic mean between Precision and Recall: $F_1 = 2 * \frac{P * R}{P + R}$. We used $F_1$ to decide the highest performing model because it balances precision and recall, which are both important in an imbalanced dataset.
    %We used $F_1$ to decide between classifiers, but the Precision and Recall scores give valuable information about the classifier's behavior.
    \item \textbf{Training time}: the wall-clock time to execute one training run with one validation run per epoch.
    \item \wip{\textbf{Inference time}: the average wall-clock time to predict for one example.}
    \item \wip{\textbf{MACs}: the average number of multiply-accumulate operations \cite{efficientnet,mobilenet} to predict for one example; this measures the performance independently of the benchmarking platform.}
% We count it as the total time to execute the program, to fairly include any extra time the approaches requires to load the dataset.
    \item \textbf{Parameter count}: the number of trainable parameters in the neural network model; this measures the model's size.
\end{itemize}

\ben{Let's move these details to appendix if we need space.}
\wip{
To measure the performance, we trained the models 3 times and reported the mean score and standard deviation for each metric.
We measured inference time and MACs on the {\bigvul} test set.
For fairness, we ran the same batch size (16, largest permissible for LineVul) for all models during runtime benchmarking.
We ran 3 warmup batches before measuring the rest of the batches to measure the average measurement per example.
We used the DeepSpeed {\needcite} profiler to measure MACs.
% 
We ran the runtime benchmarks on an AMD Ryzen 5 1600 3.2 GHz processor with 48GB of RAM and an Nvidia 3090 GPU with 24GB of GPU memory.
}
}


% Results comparing with nontransformer models
%Since transformer-based vulnerability detection models incorporate a large-scale pretraining phase, we grouped the evaluation into non-transformer-based models and transformer-based models.

% {\tool} performs significantly better than all the other baselines, except LineVul (average difference F1 between {\tool} and non-transformer-based models was 0.46).

%\wip{The 3 baselines which have higher precision unfortunately performed with a low recall, so their F1 score was significantly lower than {\tool}'s.}


\begin{mycomment}{
these graph representations cannot be used to compute dataflow information and thus may not be useful for the model to learn the causal relationship between bugs and dataflow.
and thus may not learn to represent information which is effective for vulnerability detection.
is based on domain knowledge and has a small vocabulary while the other models used unsupervised word embeddings such as Word2Vec, Doc2Vec, and GloVe, which may not learn to represent information which is effective for vulnerability detection.
\wip{Devign and ReVeal used CPG which combines AST, CFG, and PDG, while {\tool} used only the CFG. AST and PDG information are useful to detect certain classes of bugs \citep{yamaguchi_modeling_2014}, but these graph representations cannot be used to compute dataflow information and thus may not be useful for the model to learn the causal relationship between bugs and dataflow}.
}
\end{mycomment}

% CFG and abstract dataflow embedding allowed {\tool} to learn to detect vulnerabilities.

% \todo{more discussion}
% \begin{itemize}
%     \item Our model uses a simple node embedding while {\xxx} models used Word2Vec, Doc2Vec, GloVe, IVDetect used (a lot of) embeddings, which may not be effective or needed.
%     \item Our model uses only the CFG because it emulates DFA; other models use PDG and AST, which may not be effective or needed.
%     \item Compare the number of epochs to convergence with the others, and stability.
% \end{itemize}
% \end{wipenv}

% Transformer models, adding DeepDFA+LineVul

% DeepDFA

% DeepDFA+LineVul


% 


% The results of the evaluation are in Table \ref{fig:concat-comparison}.
%{\tool}'s Recall was higher than LineVul while the Precision was lower, resulting in a lower F1 score.The addition of {\tool} improved LineVul's performance in both Precision and Recall, thus increasing the F1 score by \wip{3.34 (3.6\%)}.
% There is no significant addition to runtime (+\xxx minutes) because the {\tool} encoder is small and fast to train.

% Its improvement may be caused by adding some structural and dataflow information which was missing from the transformer's token-based representation.

\begin{wipenv}
%We hypothesize that the examples which {\tool} predicted incorrectly could not be detected by reaching definitions, and that other methods of dataflow analysis may be able to detect these. \ben{need evidence to back up this point or need to make it more palatable.}
% \todo{more discussion}
% \begin{itemize}
%     \item Though our model's F1 score was lower overall, its recall was higher
%     \item We only used undersampling, but there are better techniques to handle imbalance.
%     \item Our model converged to optimal validation performance within \wip{3} epochs and did not overfit within \wip{25} epochs, while LineVul most often overfit within \wip{10} epochs of training.
% \end{itemize}
% 
% {\tool}'s balance between Precision and Recall may be changed by addressing dataset imbalance.
% We found that changing the classification boundary only improved the F1 score by 

%We used random undersampling to balance the training dataset, but there may be other techniques to handle the dataset imbalance which will result in a better balance between Precision and Recall.

% {\tool} converged within {\xxx} epochs and did not overfit, while LineVul often overfit (validation F1 started dropping) after {\xxx} epochs.
% This lends to a simpler training regime and not a lot of tricks to stop overfitting.

% \mysubsection{Discussion} \todo{write it}

% \todo{These are the total logged time from main function entry to exit. We should log only the training time.}
% \todo{FlowGNN's parameter count and training time can probably be cut while preserving performance.}
% \todo{LineVul timing are from pronto, use PC.}


% \begin{table}[h]
% \centering
% \caption{Runtime and size of the different models.
% % \todo{These are the total logged time from main function entry to exit. We should log only the training time.}
% \todo{FlowGNN's parameter count and training time can probably be cut while preserving performance.}
% % \todo{LineVul timing are from pronto, use PC.}
% }\label{fig:runtime-size-comparison}
% \begin{tabular}{|l|r|r|r|r|}
% \hline
% Model & Training time & \wip{Inference time} & \wip{MACs} & \# parameters \\
% \hline
% % VulDeePecker \\
% % SySeVR \\
% % Draper \\
% IVDetect        & \multicolumn{1}{|c|}{-} & & & 924,165 \\\hline
% Devign          & \multicolumn{1}{|c|}{-} & & & 1,148,553 \\\hline
% ReVeal          & \multicolumn{1}{|c|}{-} & & & 560,291 \\\hline
% ReGVD           & \multicolumn{1}{|c|}{-} & & & 124,794,500 \\\hline
% CodeBERT        & \multicolumn{1}{|c|}{-} & & & 124,646,401 \\\hline
% LineVul         & \wip{10h19m}  & \wip{7.23 ms} & \wip{5793.95 B} & 125,238,531  \\\hline
% {\tool}         & \wip{24m}     & \wip{1.92 ms} & \wip{40.27 M} & 375,938       \\\hline     
% {\combinedtool} & \wip{10h40m}  & \wip{7.57 ms} & \wip{5793.99 B} & 125,679,236  \\       %249,734,276
% \hline
% \end{tabular}
% \end{table}


%shows the results.We only compared the runtimes of {\tool}, LineVul, and {\combinedtool} because all other models performed significantly worse.
%

% Because of {\tool}'s small parameter count, it is ideal for resource-limited computing platforms such as mobile, AV, and embedded systems, where large pretrained transfrormers like LineVul cannot be used \citep{han_deep_2016,iandola_squeezenet_2016}.

%Both attributes enable efficient distributed training and deployment because they cut down on transfer time and time per training run.
%\end{wipenv}

% \mysubsection{Discussion}
% \todo{cleanup discussion}

% {\tool} achieved 74\% of LineVul's performance with less training time and fewer parameters.
% This is possible because {\tool} uses a more compact input representation compared to tokenized strings and propagates information along only the CFG edges, rather than associating every pair of tokens.

% {\tool}'s short training time enables techniques like per-project fine-tuning and hyperparameter tuning.
% Because of {\tool}'s small parameter count \citep{DEEP COMPRESSION, SQUEEZENET}, it is ideal for resource-restricted edge computing platforms such as mobile, AV, embedded, where large pretrained transfrormers like LineVul cannot be used.
% Both attributes enable efficient distributed training and export to devices because they cut down on transfer time and time per training run.

%\begin{wipenv}

% % \begin{minipage}
% \begin{figure}[t]
% % \begin{wrapfigure}[10]{r}{0.5\textwidth}
%     \centering
%     % \begin{spacing}{2.0}
%     \includegraphics[width=0.5\textwidth]{figures/cross-project.png}
%     \caption{Comparison of LineVul and {\combinedtool} on cross-project and mixed-project datasets.}
%     \label{fig:cross-project}
%     % \end{spacing}
% \end{figure}
% % \end{wrapfigure}
% % \end{minipage}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/bug-types.png}
%     \caption{Comparison of LineVul and {\combinedtool} on cross-bugtype and mixed-bugtype datasets.}
%     \label{fig:cross-project}
% \end{figure}


% DRAFT 1: cross-project and bug type full figures. Not very convincing.

% Figure \ref{fig:cross-project} shows the results.
% By itself, LineVul performs consistently around the median F1 = 84.16 on the mixed-project dataset.
% The performance on the cross-project dataset is lower and less consistent than mixed-project.
% In contrast, {\combinedtool} performs consistently higher at the median F1 = 87.47 on mixed-project, and performs more consistently on the cross-project dataset.
% \todo{Add more discussion when all results are in.}

% DRAFT 2: highlight the improvements of our technique.

% \mysubsection{Generalization to unseen projects}


%{\tool} performed worse than the other models (average drop of 15.53) on the mixed-project dataset, but had comparable performance with the other models (average drop of 3.03) on the cross-project test dataset. However, {\tool} had significantly more consistent performance between cross-project and mixed-project sets, with a mean drop of only 1.91 points (2.7\% drop) compared to 12.81 (15.2\% drop) for LineVul and 16.02 (18.2\% drop) for {\combinedtool}.{\combinedtool} had the best performance on the cross-project and mixed-project datasets, improving on LineVul's mean F1 score by 0.54 and 3.74 points respectively.

% Why does ours generalize better? Doesn't rely on identifier names, operators and datatypes are likely shared between projects.




\begin{comment}
\begin{wipenv}
We investigated the following RQ's in order to understand the benefit of {\tool} by itself and combined with other tools.

\begin{itemize}
    \item RQ1. Is {\tool} a useful vulnerability detection model?
    \item RQ2. How can {\tool} be used to augment transformer-based models?
\end{itemize}
% \begin{itemize}
%     \item RQ1. Is {\tool}'s dataflow analysis useful for function-level vulnerability detection?
%     \item RQ2. What is the contribution of dataflow features compared to continuous(semantic) feature representations?
%     \item RQ3. How well does {\tool} generalize to unseen projects?
%     \item RQ4. How well does {\tool} generalize to unseen bug types?
% \end{itemize}
\end{wipenv}

% \subsection{Feature Extraction}

% Epochs.
% Undersample training set.

% L2 regularization.
% Learning rate scheduler.
% Gradient clipping.
% Abstract dataflow threshold.
% GGNN parameters

% \section{Results}

\subsection{RQ1. Is {\tool} a useful vulnerability detection model?}

\begin{wipenv}
We investigated 2 parts of this RQ: generalization and runtime. \todo{justification}
% These are both important because the model should perform well and should not take a long time to train/predict.
We trained and evaluated {\tool} and baselines on the canonical train/valid/test splits of the {\dataset} and Devign datasets.

Results of the performance evaluation are shown in Table \ref{fig:performance-comparison}.
{\tool} performs significantly better than all the other baselines, except LineVul (average difference F1 between {\tool} and non-transformer-based models was 0.46).
Interestingly, {\tool}'s recall was higher than LineVul while the precision was lower, resulting in a lower F1 score.

Results for runtime and parameter count are shown in Table \ref{fig:runtime-size-comparison}. We considered only {\tool} and LineVul when reporting the training time and model size because the other models performed significantly worse.
% 
Compared to LineVul, {\tool} has significantly shorter training time (\xxx\%) and smaller parameter count (\xxx\%) and was still able to achieve 74\% of its performance.
This is possible because {\tool} uses a more compact input representation compared to tokenized strings and propagates information along only the CFG edges, rather than associating every pair of tokens.

Because of {\tool}'s short training time, it is ideal for applications like per-project fine-tuning and hyperparameter tuning.
Because of {\tool}'s small parameter count \citep{DEEP COMPRESSION, SQUEEZENET}, it is ideal to be used on resource-restricted edge computing platforms such as mobile, AV, embedded, where large pretrained transfrormers like LineVul cannot be used.
Both attributes enable efficient distributed training and export to devices because they cut down on transfer time and time per training run.

% Outline
% \begin{itemize}
%     \item 2 parts: performance and scalability.
%     \item 2 datasets: {\dataset} and Devign.
%     \item Performance
%     \item Scalability
% \end{itemize}
\end{wipenv}

\subsection{RQ2. How can {\tool} be used to augment transformer-based models?}

\begin{wipenv}
We investigated whether {\tool} could be combined with LineVul to improve the performance above the state-of-the-art.

LineVul is made of a transformer encoder and a classification layer.
We concatenated to the representation output by LineVul's transformer encoder stage the representation output by {\tool}'s graph learning stage (after the readout and before the classification layer), before feeding into the LineVul classification layer. Then, we compared the performance of the original LineVul model with the performance of the {\tool} model.
Because {\tool} uses a parser Joern which cannot parse some programs and our research prototype for extracting the abstract dataflow representation does not handle all C language features, \wip{7\%} of programs in the {\dataset} dataset could not be parsed, and to ensure a fair comparison, these were excluded from training/validation/testing for both models.
This is an artifact of our research prototype, but can be improved by introducing a better parser and improving the abstract dataflow implementation.

The results of the evaluation are in Table \ref{fig:concat-comparison}.
The addition of {\tool} improved the SOTA LineVul model in both Precision and Recall, thus increasing the F1 score by 0.0434 (5\%).
There is no significant addition to runtime (+\xxx minutes) because the {\tool} encoder is small and fast to train.

% \begin{table}
% \centering
% \caption{LineVul performance on the {\dataset} test dataset. \todo{LineVul+FlowGNN is only 1 seed}}\label{fig:concat-comparison}
% \begin{tabular}{|l|c|c|c|r|r|}
% \hline
% Model & F1 & P & R & Training runtime & \# parameters \\
% \hline
% LineVul             & 0.9158        & 0.9599        & 0.8755       & $\sim$12 hours & $\sim$250M \\\hline
% {\combinedtool}   & {\bf 0.9592}	& {\bf0.9849}	& {\bf 0.9349} & $\sim$12 hours & $\sim$250M \\
% \hline
% \end{tabular}
% \end{table}

\end{wipenv}

% \subsection{RQ3}

% Results are shown in Table \ref{fig:continuous-ablation}.

% Expected conclusions: high-ish performance, fast runtime.

% \begin{table}
% \caption{Ablation study of {\tool} vs. continuous features.}\label{fig:continuous-ablation}
% \begin{tabular}{|l|c|c|c|}
% \hline
% Features & F1 & P & R \\
% \hline
% Continuous only & huh & huh & huh \\
% Dataflow & huh & huh & huh \\
% Dataflow + Continuous & huh & huh & huh \\
% \hline
% \end{tabular}
% \end{table}

% \subsection{RQ4}

% Results are shown in Table \ref{fig:bugtype}.

% \begin{table}
% \caption{{\tool} performs best on dataflow-related bugs, significantly beating state-of-the-art.}\label{fig:bugtype}
% \begin{tabular}{|l|c|c|c||l|c|c|c|}
% \hline
% \multicolumn{4}{|c||}{BOF+NPD+ML} &
% \multicolumn{4}{|c|}{Other} \\
% \hline
% Model & F1 & P & R & Model & F1 & P & R \\
% \hline
% IVDetect & boo & dumb & low & IVDetect & boo & dumb & low \\
% LineVD & boo & dumb & low & LineVD & boo & dumb & low \\
% {\tool} & high & awesome & cool & {\tool} & high & awesome & cool \\
% \hline
% \end{tabular}
% \end{table}

\end{comment}




% \input{sections/conclusion}
\begin{comment}{
\section{Limitations and Threats}
Our research prototype could not process 7\% of the {\dataset} dataset, so these examples were excluded. In Figure \ref{fig:compare-transformer}, we reproduced the baseline approaches whose performance is comparable to {\tool} in order to make sure that the performance differences are truly due to the model changes and not the dataset changes.
This is due to the implementation of our prototype, but is separate from our research contribution.

% \subsection{External validity}

We only studied one dataset ({\dataset}),
% and only implemented one dataflow analysis (reaching definitions),
which may raise questions about the generality of our work.
To address this concern, we investigated the cross-project generalization using a different partition of the dataset.
We also studied {\tool} by itself and in combination with a transformer model, which shows that it can be used in several contexts.
% We leave other dataflow analyses for future work.
% 
\begin{wipenv}
% \todo{Cross-Bugtypes dataset}
% 
The cross-project dataset performance we reported may be affected by the choice of projects in the test set. We used 5-fold cross-validation to address this.
\end{wipenv}
}
\end{comment}

%\wip{and to explain the predictions of our model using the causal relationship of DFA and bugs}.

%With the minimum training and inference time and the model size, DeepDFA achieved the second best performance.





%\wip{Our experimental results confirm that {\tool} is performant and efficient, and generalizes better, than other models.}



% Future work:
% \begin{itemize}
%     \item other dataflow analyses
%     \item other abstract interpretation
%     \item explanation based on dataflow analysis
%     \item improve abstract dataflow representation
% \end{itemize}
% \end{wipenv}




